Dolma: an Open Corpus of Three Trillion Tokens for Language Model Pretraining Research

Information about pretraining corpora used to train the current best-performing language models is seldom discussed: commercial models rarely detail their data, and even open models are often released without accompanying training data or recipes to reproduce them. As a result, it is challenging to conduct and advance scientific research on language modeling, such as understanding how training data impacts model capabilities and limitations. To facilitate scientific research on language model pretraining, we curate and release Dolma, a three-trillion-token English corpus, built from a diverse mixture of web content, scientific papers, code, public-domain books, social media, and encyclopedic materials. We extensively document Dolma, including its design principles, details about its construction, and a summary of its contents. We present analyses and experimental results on intermediate states of Dolma to share what we have learned about important data curation practices. Finally, we open-source our data curation toolkit to enable reproduction of our work as well as support further research in large-scale data curation.

==> 5-releasing.tex <==

\section{Releasing Dolma}
\label{sec:release}

\ye{this can be renamed as ethics section, and then we get unlimited space for this part}


\paragraph{Risk mitigation} We recognize that any dataset derived from large web crawls will contain factually incorrect information, toxic language, hate speech, PII, and other types of harmful content. 
While we have made an effort to curate this dataset taking this into consideration, we believe risk mitigation is best approached from multiple directions,
including careful consideration of licenses and access controls.






\paragraph{Copyright} While most datasets we used were curated with copyright and licensing in mind (e.g., open access papers in peS2o~\citep{peS2o}, open source repositories in the Stack~\citep{kocetkov2022stack}) or were already permissively licensed (e.g., Wikipedia is released under a Creative Commons license), we recognize that large web crawls will also contain copyrighted material. 
Yet, given current tools, it's not possible to reliably or scalably detect copyrighted materials in a corpus of this size.
Our decision to release \dolma publicly factors in several considerations, including that all our data sources were publicly available and already being used in large-scale language model pretraining (both open and closed), we refer the reader to our public position on AI and fair use~\citep{uspto-copyright-ai2}.

We recognize that the legal and ethical landscape of AI is changing rapidly, and we plan to revisit our choices as new information becomes available.

